A backward procedure for change-point detection with applications to copy number variation detection

Change-point detection regains much attention recently for analyzing array or sequencing data for copy number variation (CNV) detection. In such applications, the true signals are typically very short and buried in the long data sequence, which makes it challenging to identify the variations efficiently and accurately. In this article, we propose a new change-point detection method, a backward procedure, which is not only fast and simple enough to exploit high-dimensional data but also performs very well for detecting short signals. Although motivated by CNV detection, the backward procedure is generally applicable to assorted change-point problems that arise in a variety of scientific applications. It is illustrated by both simulated and real CNV data that the backward detection has clear advantages over other competing methods especially when the true signal is short.

==> tb_level2.tex <==
\begin{table} [htbp] 
\begin{center}
\begin{tabular}{cccccccc}
\hline
\multicolumn{2}{l}{} & &\multicolumn{3}{c}{Normal}            & \multicolumn{2}{c}{t} \\
\multicolumn{2}{l}{Methods} & $\alpha$ &    $n=1000$ &  $n=3000$ &	$n=5000$ &	  df$ = 10$ &     df$= 5$ \\ \hline
\multirow{4}*{BWD}
&\multirow{2}*{cutoff1}
 &0.01   &	.011 &	.013 & 	.009 &	.032 &	.030 \\
&&0.05   &	.051 &	.046 & 	.058 &	.077 &	.065 \\ \cline{2-8}
&\multirow{2}*{cutoff2}
&0.01   &	.014 &	.018 & 	.010 &	.007 &	.002 \\
&&0.05   &	.065 &	.070 &	.053 &	.052 &	.022 \\ \hline
\multicolumn{2}{c}{CBS} &N/A&    .007&	.011& 	.010& 	.003&	.003 \\
\multicolumn{2}{c}{WBS} &N/A&    .016&	.005& 	.004& 	.112&	.395\\
\multicolumn{2}{c}{LRS} &N/A&    .022&	.028& 	.028& 	.388&	.905 \\
\multicolumn{2}{c}{TGUH}&N/A&    .030&	.023& 	.019& 	.098&	.210 \\ \hline
\end{tabular}
\end{center}
\caption{Estimated level - The cutoff1 performs well under normality assumption is true and the cutoff2 can be used if the normality assumption is suspicious.} \label{tb::level}
\end{table}


==> tb_normal2.tex <==
\begin{table}[htbp] 
\begin{center}
\begin{tabular}{cccc ccccc ccccc cc}
\hline
    &\multicolumn{2}{c}{$L$}      &\multicolumn{6}{c}{5} & \multicolumn{6}{c}{10} \\
    &\multicolumn{2}{c}{$\delta$} &\multicolumn{2}{c}{1.5} & \multicolumn{2}{c}{2.0} & \multicolumn{2}{c}{2.5} &
               \multicolumn{2}{c}{1.5} & \multicolumn{2}{c}{2.0} & \multicolumn{2}{c}{2.5} \\
$n$ &\multicolumn{2}{c}{Methods}& Sen. & Pre. & Sen. & Pre. & Sen. & Pre. & Sen. & Pre. & Sen. & Pre. & Sen. & Pre. \\ \hline
\multirow{8}*{1,000} &
  \multirow{2}*{BWD1}
     & .01 & .183  & .948	& .571	& .976	& .904	& .992	& .639	& .983	& .960	& .993	& .998	& .994\\
&   & .05 & .334	& .817	& .724	& .916	& .951	& .945	& .768	& .924	& .982	& .944	& .999	& .952\\
&\multirow{2}*{BWD2}
     & .01 & .190	& .941	& .591	& .982	& .900	& .988	& .658	& .981	& .964	& .992	& .999	& .993\\
&   & .05 & .335	& .831	& .746	& .912	& .946	& .940	& .785	& .906	& .986	& .939	& .999	& .949\\ \cline{2-15}
&\multicolumn{2}{c}{CBS}
      &  .165 	& .948 	& .555 	& .975 	& .900 	& .979 & .648 	& .972 	& .972 	& .976 	& .999 	& .977\\
&\multicolumn{2}{c}{WBS}
      &   .176 & .884	& .570	& .942	& .909	& .954 & .634 	& .948 	& .971 	& .956 	& .999 	& .957\\
&\multicolumn{2}{c}{LRS}
      & .216   & .911 	& .638 	& .973 	& .942 	& .983 & .701 	& .979 	& .984 	& .988 	&1.000 	& .989\\ %\cline{2-11}
&\multicolumn{2}{c}{TGUH}
      & .053   & .546 	& .079 &  .603 &  .090  & .657 & .217   & .804 	& .233  & .809 	& .240  & .805\\ \hline %\cline{2-11}

\multirow{8}{9mm}{3,000} &
  \multirow{2}*{BWD1}
     & .01 & .132	& .961	& .509	& .990	& .869	& .995	& .562	& .991	& .958	& .995	& .999	& .992\\
&   & .05 & .267	& .885	& .688	& .958	& .938	& .974	& .731	& .963	& .983	& .974	& .999	& .998\\
&\multirow{2}*{BWD2}
     & .01 & .140	& .970	& .525	& .991	& .873	& .995	& .569	& .990	& .959	& .995	& .999	& .996\\
&   & .05 & .279	& .884	& .708	& .949	& .942	& .968	& .749	& .940	& .983	& .964	& .999	& .998\\ \cline{2-15}
&\multicolumn{2}{c}{CBS}
               & .103 	& .960 	& .490 	& .984 	& .882 	& .985 & .572 	& .983 	& .974 	& .982 	& .999 	& .983 \\
&\multicolumn{2}{c}{WBS}
         	   & .079  	& .967 	& .399 	& .991 	& .819  & .990 & .470 	& .991 	& .938 	& .992 	& .999  & .990\\
&\multicolumn{2}{c}{LRS}
               & .152 	& .948 	& .553 	& .986 	& .898 	& .993 & .606 	& .988 	& .972 	& .994 	& .999 	& .996 \\ 
&\multicolumn{2}{c}{TGUH}
               & .016   & .623 	& .048  & .883 	& .056  & .960 & .099   & .934 	& .139  & .965 	& .129  & .967\\ \hline %\cline{2-11}

\multirow{8}*{5,000} &
  \multirow{2}*{BWD1}
     & .01 & .113	& .966	& .477	& .995	& .859	& .997	& .526	& .991	& .944	& .995	& .999	& .996\\
&   & .05 & .241	& .926	& .670	& .975	& .935	& .986	& .701	& .973	& .978	& .983	& .999	& .986\\
&\multirow{2}*{BWD2}
     & .01  & .120	& .974	& .490	& .995	& .869	& .996	& .545	& .993	& .946	& .996	& .999	& .997\\
&   & .05  & .254	& .913	& .686	& .972	& .938	& .979	& .721	& .962	& .979	& .982	& .999	& .983\\ \cline{2-15}
&\multicolumn{2}{c}{CBS}
               & .088 	& .973 	& .468 	& .989 	& .890 	& .987 & .551 	& .983 	& .966 	& .985 	&1.000 	& .987\\
&\multicolumn{2}{c}{WBS}
               & .052  	& .985	& .327 	& .994 	& .730 	& .995 & .383  	& .994 	& .891 	& .995 	& .997 	& .995\\
&\multicolumn{2}{c}{LRS}
               & .130 	& .962 	& .512 	& .992 	& .881 	& .996 & .563 	& .992 	& .957 	& .997 	& .999 	& .997\\ 
&\multicolumn{2}{c}{TGUH}
               & .010   & .722 	& .035  & .951 	& .043  & .995 & .076   & .974 	& .091  & .991 	& .087  & .991\\ \hline
\end{tabular}
\end{center}
\caption{Performances under normal error - The BWD and LRS outperform others. The backward detection with $\alpha = .05$ ($.01$) shows higher (lower) sensitivity but lower (higher) precision compared to the LRS. TGUH does not perform well for detecting short signals. } \label{tb::normal}
\end{table}


==> tb_t2.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{ccc ccccc ccc} 
\hline
    \multicolumn{2}{c}{$L$}      &\multicolumn{4}{c}{5} & \multicolumn{4}{c}{10}\\
    \multicolumn{2}{c}{$df$} &\multicolumn{2}{c}{10} & \multicolumn{2}{c}{5} &
                              \multicolumn{2}{c}{10} & \multicolumn{2}{c}{5} \\
\multicolumn{2}{c}{Methods}& Sen. & Pre. & Sen. & Pre. & Sen. & Pre. & Sen. & Pre.\\ \hline
\multirow{2}*{BWD1}
     & .01 & .932	& .990	& .589	& .982	& 1.000	& .993	& .968	& .983\\
     & .05 & .965	& .949	& .879	& .879	& 1.000	& .952	& .994	& .942\\
\multirow{2}*{BWD2}
     & .01 & .936	& .993	& .606	& .985	& 1.000	& .996	& .967	& .986\\
     & .05 & .969	& .952	& .876	& .893	& 1.000	& .958	& .993	& .954\\
\multicolumn{2}{c}{CBS}
               & .853 	&.987 	&.287 	&.986 &  .998 	&.986 	&.864 	&.990\\
\multicolumn{2}{c}{WBS}
               &.981    &.867   &.939 	&.644 & 1.000   &.865   &.999   &.651\\
\multicolumn{2}{c}{LRS}
               & .983 	&.711 	&.907 	&.338 & 1.000 	&.741 	&.999 	&.375\\ 
\multicolumn{2}{c}{TGUH}
               & .273   &.720 	&.545   &.619 &  .391   &.752 	&.699   &.666\\ \hline
\end{tabular}
\end{center}
\caption{Performances under t-distributed error - The BWD outperforms all other methods for detecting short signals. } \label{tb::t}
\end{table}


